Rigidity Preserving Image Transformations and Equivariance in Perspective

We characterize the class of image plane transformations which realize rigid camera motions and call these transformations `rigidity preserving'. In particular, 2D translations of pinhole images are not rigidity preserving. Hence, when using CNNs for 3D inference tasks, it can be beneficial to modify the inductive bias from equivariance towards translations to equivariance towards rigidity preserving transformations. We investigate how equivariance with respect to rigidity preserving transformations can be approximated in CNNs, and test our ideas on both 6D object pose estimation and visual localization. Experimentally, we improve on several competitive baselines.

==> tables/lm_aggregated_poster.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW RESULTS FOR ICML - MEDIANS FOR 3X RERUNS, AND INCLUDING NEW SOTA: DFPN-6D
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline

% Hack solution of citations for AAAI style
EP: Baseline
& EP: $\PY$
& EP: $\Hm_{\mathrm{aug}}$

% & DPOD+\footnote{Zakharov et al., ICCV 2019.}
& PVNet\footnote{Peng et al., CVPR 2019.}
& HybridPose\footnote{Song et al., CVPR 2020.}
% & CDPN\footnote{Li et al., ICCV 2019.}
& BPnP\footnote{Chen et al., CVPR 2020.}
& DFPN-6D\footnote{Cheng et al., IEEE Trans. Instrum. Meas. 2021.}

% % & DPOD+\footnote{Zakharov et al. (ICCV 2019)}
% & PVNet\footnote{Peng et al. (CVPR 2019)}
% & HybridPose\footnote{Song et al. (CVPR 2020)}
% % & CDPN\footnote{Li et al. (ICCV 2019)}
% & BPnP\footnote{Chen et al. (CVPR 2020)}
% & DFPN-6D\footnote{Cheng et al. (IEEE Trans. Instrum. Meas. 2021)}

% % & DPOD+\footnote{Zakharov et al. (2019)}
% & PVNet\footnote{Peng et al. (2019)}
% & HybridPose\footnote{Song et al. (2020)}
% % & CDPN\footnote{Li et al. (2019)}
% & BPnP\footnote{Chen et al. (2020)}
% & DFPN-6D\footnote{Cheng et al. (2021)}

% & PVNet\tnote{1}
% & HybridPose\tnote{2}
% & BPnP\tnote{3}
% & DFPN-6D\tnote{4}
\bigstrut
\\

% $^1$ Zakharov et al. (ICCV 2019),
% $^2$ Peng et al. (CVPR 2019),
% $^3$ Song et al. (CVPR 2020),
% % $^4$ Li et al. (ICCV 2019),
% $^4$ Chen et al. (CVPR 2020),
% $^5$ Cheng et al. (IEEE Trans. Instrum. Meas. 2021).

\hline
\result{95.56} (\result{97.35})
% & \oldwrongcell \result{97.09} % PY phi=0, old, rot ref target: cam
& \newcorrectcell \result{97.43} % PY phi=0, rot ref target: aligned2obj
& \result{97.21}
% & \result{95.15} % DPOD not prioritized: (somewhat unfair advantage in refinement step)
& \result{86.27} % PVNet not prioritized: Not very competitive anymore
& \result{94.50}
% & \result{89.86} % CDPN not prioritized: Not very competitive
& \result{93.27}
& \resultbf{98.06}
\bigstrut
\\

\hline
\end{tabular}

% $^1$ Zakharov et al. (ICCV 2019),
% $^2$ Peng et al. (CVPR 2019),
% $^3$ Song et al. (CVPR 2020),
% % $^4$ Li et al. (ICCV 2019),
% $^4$ Chen et al. (CVPR 2020),
% $^5$ Cheng et al. (IEEE Trans. Instrum. Meas. 2021).

% $^1$\cite{Zakharov_2019_ICCV},
% $^2$\cite{Peng_2019_CVPR},
% $^3$\cite{Song_2020_CVPR},
% % $^4$\cite{Li_2019_ICCV},
% $^4$\cite{Chen_2020_CVPR},
% $^5$\cite{Cheng_2021_IEEETransInstrumMeas}.






==> tables/lm_aggregated_presentation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW RESULTS FOR ICML - MEDIANS FOR 3X RERUNS, AND INCLUDING NEW SOTA: DFPN-6D
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline

\multicolumn{4}{|c|}{\EP{} ($\phi=0$)}
& \multicolumn{4}{c|}{Competing methods}
% \bigstrut
\\
\hline
% Hack solution of citations for AAAI style
\eporigcell Original
& Baseline
& \ourscell $\PY$
& \ourscell $\Hm_{\mathrm{aug}}$
% & DPOD+$^1$
& PVNet$^1$
% & HybridPose$^2$
% & CDPN$^4$
& BPnP$^2$
% & RePOSE$^3$%\cite{Iwase_2021_ICCV}
& RNNPose$^3$%\cite{xu2022rnnpose}
& DFPN-6D$^4$
% \bigstrut
\\
% \hline
% % Hack solution of citations for AAAI style
% \eporigcell EP: Original
% & EP: Baseline
% & \ourscell EP: $\PY$
% & \ourscell EP: $\Hm_{\mathrm{aug}}$
% % & DPOD+$^1$
% & PVNet$^1$
% & HybridPose$^2$
% % & CDPN$^4$
% & BPnP$^3$
% & DFPN-6D$^4$
% % \bigstrut
% \\
\hline
% \result{95.56} (\result{97.35})
% \eporigcell
\textcolor{fg!40}{
(\result{97.35})
}
& \result{95.56}
&
% \ourscell
% \oldwrongcell \result{97.09} % PY phi=0, old, rot ref target: cam
\newcorrectcell \result{97.43} % PY phi=0, rot ref target: aligned2obj
&
% \ourscell
\result{97.21}
% & \result{95.15} % DPOD not prioritized: (somewhat unfair advantage in refinement step)
& \result{86.27} % PVNet not prioritized: Not very competitive anymore
& \result{94.50}
% & \result{89.86} % CDPN not prioritized: Not very competitive
& \result{93.27}
& \resultbf{98.06}
% \bigstrut
\\

\hline
\end{tabular}
\\
{\smaller
% $^1$ Zakharov et al. (2019),
$^1$ Peng et al. (2019),
% $^2$ Song et al. (2020),
% $^4$ Li et al. (2019),
$^2$ Chen et al. (2020),
$^3$ Xu et al. (2022),
$^4$ Cheng et al. (2021).
}

% $^1$ Zakharov et al. (ICCV 2019),
% $^2$ Peng et al. (CVPR 2019),
% $^3$ Song et al. (CVPR 2020),
% % $^4$ Li et al. (ICCV 2019),
% $^4$ Chen et al. (CVPR 2020),
% $^5$ Cheng et al. (IEEE Trans. Instrum. Meas. 2021).

% $^1$\cite{Zakharov_2019_ICCV},
% $^2$\cite{Peng_2019_CVPR},
% $^3$\cite{Song_2020_CVPR},
% % $^4$\cite{Li_2019_ICCV},
% $^4$\cite{Chen_2020_CVPR},
% $^5$\cite{Cheng_2021_IEEETransInstrumMeas}.


==> tables/occl_aggregated_poster.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW RESULTS FOR ICML - MEDIANS FOR 3X RERUNS
\begin{tabular}{|c|c|c|c||c|c|c|c|}
    \hline
    \multicolumn{4}{|c||}{$\phi=0$}
        & \multicolumn{4}{c|}{$\phi=3$}

        \bigstrut
        \\
     \hline
    % Object
        %  &
         Original
         &
         Baseline
        %  $\mathbb{P}^2$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $180^\circ$
        %     }
        % }
         &
         $\PY$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\PY$\\ Roll $180^\circ$
        %     }
        % }
         &
         $\Hm_{\mathrm{aug}}$
        %  $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
        %     }
        % }
         &
         Original
         &
         Baseline
        %  $\mathbb{P}^2$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $180^\circ$
        %     }
        % }
         &
         $\PY$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\PY$\\ Roll $180^\circ$
        %     }
        % }
         &
         $\Hm_{\mathrm{aug}}$
        %  $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
        %     }
        % }

        \bigstrut
                 \\
    \hline
   \result{79.04} % phi=0 Original
       & \result{77.44} % phi=0 Baseline
    %   & \oldwrongcell \result{80.47} % PY phi=0, old, rot ref target: cam
        & \newcorrectcell \result{80.43} % PY phi=0, rot ref target: aligned2obj
       & \result{83.58} % phi=0 RHaug
       & \result{83.98} % phi=3 Original
       & \result{81.94} % phi=3 Baseline
       & \result{82.91} % phi=3 PY
       & \resultbf{84.92} % phi=3 RHaug
      \bigstrut
       \\
    \hline
\end{tabular}


==> tables/occl_aggregated_presentation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW RESULTS FOR ICML - MEDIANS FOR 3X RERUNS
\begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    % \multicolumn{4}{|c|}{$\phi=0$}
    %     & \multicolumn{4}{c|}{$\phi=3$}
    \multicolumn{4}{|c|}{\EP{} ($\phi=0$)}
        & \multicolumn{4}{c|}{\EP{} ($\phi=3$)}

        % \bigstrut
        \\
     \hline
    % Object
        %  &
         \eporigcell
         Original
         &
         Baseline
        %  $\mathbb{P}^2$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $180^\circ$
        %     }
        % }
         &
         \ourscell
         $\PY$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\PY$\\ Roll $180^\circ$
        %     }
        % }
         &
         \ourscell
         $\Hm_{\mathrm{aug}}$
        %  $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
        %     }
        % }
         &
         \eporigcell
         Original
         &
         Baseline
        %  $\mathbb{P}^2$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $180^\circ$
        %     }
        % }
         &
         \ourscell
         $\PY$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\PY$\\ Roll $180^\circ$
        %     }
        % }
         &
         \ourscell
         $\Hm_{\mathrm{aug}}$
        %  $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
        %  \rottableheader{
        %     \parbox{3cm}{
        %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
        %     }
        % }

        % \bigstrut
                 \\
    \hline
%   \eporigcell
\textcolor{fg!40}{
   (\result{79.04}) % phi=0 Original
}
       & \result{77.44} % phi=0 Baseline
       &
    %   \ourscell
    %   \oldwrongcell \result{80.47} % PY phi=0, old, rot ref target: cam
        \newcorrectcell \result{80.43} % PY phi=0, rot ref target: aligned2obj
       &
    %   \ourscell
        % \result{81.92} % phi=0 RHaug, roll=180
        \result{83.58} % phi=0 RHaug, roll=45
       &
    %   \eporigcell
\textcolor{fg!40}{
       (\result{83.98}) % phi=3 Original
}
       & \result{81.94} % phi=3 Baseline
       &
    %   \ourscell
       \result{82.91} % phi=3 PY
       &
    %   \ourscell
       % \resultbf{85.20} % phi=3 RHaug, roll 180
       \resultbf{84.92} % phi=3 RHaug, roll 45
    %   \bigstrut
       \\
    \hline
\end{tabular}


==> tables/old_unused/depthrot_targets_lmo.tex <==
\newcounter{tablerow}

% \begin{tabular}{|c|c|p{0.18\textwidth}|p{0.09\textwidth}|c|c|c|c|}
\begin{tabular}{
    | >{\centering\arraybackslash}m{0.07\textwidth}
    % | c
    | >{\centering\arraybackslash}m{0.024\textwidth}
    | >{\centering\arraybackslash}m{0.19\textwidth}
    | >{\centering\arraybackslash}m{0.09\textwidth}
    | >{\centering\arraybackslash}m{0.05\textwidth}
    | >{\centering\arraybackslash}m{0.10\textwidth}
    | >{\centering\arraybackslash}m{0.08\textwidth}
    | >{\centering\arraybackslash}m{0.10\textwidth}
|}
    \hline
    Image domain
        & Exp. \textnumero
        % & $x_2$ axis of Rot target frame of reference
        & Rot. target frame of reference: $x_2$ aligned with \dots
        & Depth target
        % & \#Epochs
        % & \reproj{}
        % & \degcm{}
        & \add{}
        & Avg rot error & Avg transl error
        \bigstrut
        \\
     \hline
     \multirow{3}{*}[-1.3em]{\footnotesize$\mathbb{P}^2$}
        & 1
        % & \refstepcounter{tablerow}\thetablerow
        & \gcell{} optical axis
        & \gcell{} $t_2$
        % & 5000
        % & \resultbf{77.77}
        % & \result{61.81}
        & \resultbf{79.11}
        & \resultdeg{12.96}
        & \resultbfmm{10.67}
        \bigstrut
        \\
     \cline{2-8}
    %  $\mathbb{P}^2$
        & 2
        % & \refstepcounter{tablerow}\thetablerow
        & \rcell{} per-pixel viewing ray
        & \gcell{} $t_2$
        % & 5000
        % & \result{76.65}
        % & \result{57.19}
        & \result{78.57}
        & \resultdeg{13.61}
        & \resultmm{10.83}
        \bigstrut
        \\
    %  \cline{2-8}
    % %  $\mathbb{P}^2$
    %     & 3a
    %     % & \refstepcounter{tablerow}\thetablerow
    %     & \gcell{} optical axis
    %     & \rcell{} cam-to-object distance
    %     & 5000 (old)
    %     % & \result{76.89}
    %     % & \result{61.26}
    %     & \result{77.61}
    %     & \resultdeg{13.13}
    %     & \resultmm{10.98}
    %     \bigstrut
    %     \\
    %  \cline{2-8}
    %     & 3b
    %     % & \refstepcounter{tablerow}\thetablerow
    %     & \gcell{} optical axis
    %     & \rcell{} cam-to-object distance
    %     & 7000 (old)
    %     % & \result{77.59}
    %     % & \resultbf{65.14}
    %     & \result{78.72}
    %     & \resultbfdeg{12.81}
    %     & \resultbfmm{10.55}
    %     \bigstrut
    %     \\
     \cline{2-8}
        & 3
        % & \refstepcounter{tablerow}\thetablerow
        & \gcell{} optical axis
        & \rcell{} cam-to-object distance
        % & 5000
        % & \result{77.96}
        % & \result{64.69}
        & \result{78.08}
        & \resultbfdeg{12.60}
        & \resultmm{11.10}
        \bigstrut
        \\
    %  \cline{2-8}
    %     & 3b
    %     % & \refstepcounter{tablerow}\thetablerow
    %     & \gcell{} optical axis
    %     & \rcell{} cam-to-object distance
    %     & 10000
    %     % & \result{77.97}
    %     % & \result{64.89}
    %     & \result{77.98}
    %     & \resultdeg{12.61}
    %     & \resultmm{11.16}
    %     \bigstrut
    %     \\
    %  \hline
     \hhline{|=|=|=|=|=|=|=|=|}
     \multirow{3}{*}[-1.0em]{\footnotesize$\PY$}
        & 4
        % & \refstepcounter{tablerow}\thetablerow
        & \gcell{} per-pixel viewing ray
        & \gcell{} cam-to-object distance
        % & 5000
        % & \resultbf{77.41}
        % & \resultbf{65.40}
        & \result{80.54}
        & \resultbfdeg{12.52}
        & \resultbfmm{10.19}
        \bigstrut
        \\
     \cline{2-8}
    %  $\PY$
        & 5
        % & \refstepcounter{tablerow}\thetablerow
        & \rcell{} optical axis
        & \gcell{} cam-to-object distance
        % & 5000
        % & \result{75.89}
        % & \result{61.13}
        & \resultbf{80.88}
        & \resultdeg{13.10}
        & \resultmm{10.21}
        \bigstrut
        \\
    %  \cline{2-8}
    % %  $\PY$
    %     & 6a
    %     % & \refstepcounter{tablerow}\thetablerow
    %     & \gcell{} per-pixel viewing ray
    %     & \rcell{} $t_2$
    %     & 5000 (old)
    %     % & \result{74.76}
    %     % & \result{53.10}
    %     & \result{78.61}
    %     & \resultdeg{14.06}
    %     & \resultmm{10.68}
    %     \bigstrut
    %     \\
    %  \cline{2-8}
    %     & 6b
    %     % & \refstepcounter{tablerow}\thetablerow
    %     & \gcell{} per-pixel viewing ray
    %     & \rcell{} $t_2$
    %     & 7000 (old)
    %     % & \result{76.68}
    %     % & \result{60.17}
    %     & \result{78.96}
    %     & \resultdeg{13.29}
    %     & \resultmm{10.72}
    %     \bigstrut
    %     \\
     \cline{2-8}
        & 6
        % & \refstepcounter{tablerow}\thetablerow
        & \gcell{} per-pixel viewing ray
        & \rcell{} $t_2$
        % & 5000
        % & \result{75.82}
        % & \result{63.04}
        & \result{79.13}
        & \resultdeg{13.17}
        & \resultmm{10.79}
        \bigstrut
        \\
    %  \cline{2-8}
    %     & 6b
    %     % & \refstepcounter{tablerow}\thetablerow
    %     & \gcell{} per-pixel viewing ray
    %     & \rcell{} $t_2$
    %     & 10000
    %     % & \result{75.69}
    %     % & \result{63.19}
    %     & \result{79.12}
    %     & \resultdeg{13.15}
    %     & \resultmm{10.79}
    %     \bigstrut
    %     \\
     \hline
\end{tabular}



% \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     Image domain
%         & $x_2$ axis of rotation target frame of reference
%         & \reproj{} & \degcm{} & \add{} \\
%      \hline
%      $\mathbb{P}^2$
%         & optical axis
%         & \result{77.36} & \result{62.01} & \result{79.11} \\
%      \hline
%      $\mathbb{P}^2$
%         & cam-to-object viewing ray
%         & \result{76.65} & \result{57.19} & \result{78.57} \\
%      \hline
%      $\PY$
%         & optical axis
%         & \result{75.89} & \result{61.13} & \result{80.88} \\
%      \hline
%      $\PY$
%         & cam-to-object viewing ray
%         & \result{77.41} & \result{65.40} & \result{80.54} \\
%      \hline
% \end{tabular}


==> tables/old_unused/lm_5deg5cm_perobj.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Object
         & \rottableheader{DPOD \cite{Zakharov_2019_ICCV}}
         & \rottableheader{DPOD+ \cite{Zakharov_2019_ICCV}}
         & \rottableheader{PVNet \cite{Peng_2019_CVPR}}
         & \rottableheader{HybridPose \cite{Song_2020_CVPR}}
         & \rottableheader{CDPN \cite{Li_2019_ICCV}}
         & \rottableheader{BPnP \cite{Chen_2020_CVPR}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\ $\mathbb{P}^2$, Roll $180^\circ $}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\$\PY$, Roll $180^\circ$}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\$\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$}}
         \\
     \hline
     ape
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     benchvise
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     cam
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     can
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     cat
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     driller
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     duck
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     eggbox
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     glue
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     holepuncher
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     iron
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     lamp
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     phone
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     Average
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
\end{tabular}


==> tables/old_unused/lm_adds_perobj.tex <==
    %  \rottableheader{\parbox{3cm}{\EP{}:\\$\mathbb{P}^2$, Roll $180^\circ$}}
    %  \rottableheader{\parbox{3cm}{\EP{}:\\$\PY$, Roll $180^\circ$}}
    %  \rottableheader{\parbox{3cm}{\EP{}:\\$\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$}}
    %  \rottableheader{DPOD \cite{Zakharov_2019_ICCV}}
    %  \rottableheader{DPOD+ \cite{Zakharov_2019_ICCV}}
    %  \rottableheader{PVNet \cite{Peng_2019_CVPR}}
    %  \rottableheader{HybridPose \cite{Song_2020_CVPR}}
    %  \rottableheader{CDPN \cite{Li_2019_ICCV}}
    %  \rottableheader{BPnP \cite{Chen_2020_CVPR}}
    % %  \rottableheader{$\mathbb{P}^2$, Roll $180^\circ$}
    % %  \rottableheader{$\PY$, Roll $180^\circ$}
    % %  \rottableheader{$\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Object
         & \rottableheader{DPOD \cite{Zakharov_2019_ICCV}}
         & \rottableheader{DPOD+ \cite{Zakharov_2019_ICCV}}
         & \rottableheader{PVNet \cite{Peng_2019_CVPR}}
         & \rottableheader{HybridPose \cite{Song_2020_CVPR}}
         & \rottableheader{CDPN \cite{Li_2019_ICCV}}
         & \rottableheader{BPnP \cite{Chen_2020_CVPR}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\ $\mathbb{P}^2$, Roll $180^\circ$}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\$\PY$, Roll $180^\circ$}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\$\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$}}
         \\
     \hline
     ape
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     benchvise
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     cam
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     can
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     cat
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     driller
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     duck
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     eggbox
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     glue
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     holepuncher
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     iron
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     lamp
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     phone
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     Average
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
\end{tabular}







    % \iffalse
    % \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    %     \hline
    %     Experiment setting
    %         & ape & benchvise & cam & can & cat & driller & duck & eggbox & glue & holepuncher & iron & lamp & phone & Total \\
    %      \hline
    %      \EP{}: $\mathbb{P}^2$, Roll $180^\circ$
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} (\result{97.35}) \\
    %      \hline
    %      \EP{}: $\PY$, Roll $180^\circ$
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} \\
    %      \hline
    %      \EP{}: $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} \\
    %      \hline
    %      DPOD \cite{Zakharov_2019_ICCV}
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & -- & -- & \result{82.98} \\
    %      \hline
    %      DPOD+ \cite{Zakharov_2019_ICCV}
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & -- & -- & \result{95.15} \\
    %      \hline
    %      PVNet \cite{Peng_2019_CVPR}
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{99.00} & -- & \result{86.27} \\
    %      \hline
    %      HybridPose \cite{Song_2020_CVPR}
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & -- & -- & \result{94.5} \\
    %      \hline
    %      CDPN \cite{Li_2019_ICCV}
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{98.10} & \result{94.31} & \result{89.86} \\
    %      \hline
    %      BPnP \cite{Chen_2020_CVPR}
    %         & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{} & \result{99.21} & -- & \result{93.27} \\
    %      \hline
    % \end{tabular}
    % % & \reproj{} & \degcm{} & \add{} \\
    % \fi




==> tables/old_unused/lm_reproj_perobj.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Object
         & \rottableheader{DPOD \cite{Zakharov_2019_ICCV}}
         & \rottableheader{DPOD+ \cite{Zakharov_2019_ICCV}}
         & \rottableheader{PVNet \cite{Peng_2019_CVPR}}
         & \rottableheader{HybridPose \cite{Song_2020_CVPR}}
         & \rottableheader{CDPN \cite{Li_2019_ICCV}}
         & \rottableheader{BPnP \cite{Chen_2020_CVPR}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\ $\mathbb{P}^2$, Roll $180^\circ$}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\$\PY$, Roll $180^\circ$}}
         & \rottableheader{\parbox{3cm}{\EP{}, $\phi=3$:\\$\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$}}
         \\
     \hline
     ape
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     benchvise
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     cam
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     can
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     cat
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     driller
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     duck
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     eggbox
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     glue
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     holepuncher
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     iron
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     lamp
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     phone
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
     Average
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        & \result{}
        \\
     \hline
\end{tabular}


==> tables/old_unused/lm_results_presentation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{|l||r|r|r|r|}
    \hline
     & & &  & \\
    Object & \multicolumn{1}{l|}{Original} & \multicolumn{1}{l|}{Baseline} & \multicolumn{1}{l|}{$\PY$} & \multicolumn{1}{l|}{$\Hm_\mathrm{aug}$} \bigstrut\\
    \hline
    ape
        & \result{87.71}
        & \result{80.57}
        & \result{85.43}
        & \result{88.48}
    \bigstrut\\
    \hline
    benchvise
        & \result{99.71}
        & \result{99.52}
        & \resultbf{99.90}
        & \resultbf{99.90}
    \bigstrut\\
    \hline
    cam
        & \result{97.94}
        & \result{95.20}
        & \result{97.94}
        & \result{96.76}
    \bigstrut\\
    \hline
    can
        & \result{98.52}
        & \result{98.23}
        & \result{98.82}
        & \result{99.41}
    \bigstrut\\
    \hline
    cat
        & \result{98.00}
        & \result{95.11}
        & \result{98.10}
        & \resultbf{98.90}
    \bigstrut\\
    \hline
    driller
        & \resultbf{99.90}
        & \result{99.41}
        & \result{99.60}
        & \result{99.60}
    \bigstrut\\
    \hline
    duck
        & \resultbf{90.99}
        & \result{84.13}
        & \result{89.30}
        & \result{87.70}
    \bigstrut\\
    \hline
    eggbox
        & \resultbf{100.00}
        & \resultbf{100.00}
        & \result{99.91}
        & \resultbf{100.00}
    \bigstrut\\
    \hline
    glue
        & \resultbf{100.00}
        & \result{99.90}
        & \result{99.90}
        & \resultbf{100.00}
    \bigstrut\\
    \hline
    holepuncher
        & \result{95.15}
        & \result{93.34}
        & \resultbf{97.05}
        & \result{95.53}
    \bigstrut\\
    \hline
    iron
        & \result{99.69}
        & \result{98.88}
        & \result{99.49}
        & \resultbf{100.00}
    \bigstrut\\
    \hline
    lamp
        & \resultbf{100.00}
        & \result{99.71}
        & \result{99.90}
        & \resultbf{100.00}
    \bigstrut\\
    \hline
    phone
        & \result{97.98}
        & \result{97.41}
        & \result{98.27}
        & \result{98.17}
    \bigstrut\\
    % \hline
    \hhline{|=====|}
    Average
        & \resultbf{97.35}
        & \result{95.56}
        & \result{97.09}
        & \result{97.21}
    \bigstrut\\
    \hline
\end{tabular}
\uncover<2->{
\begin{tabular}{|r|}
    \hline
    \multicolumn{1}{|l|}{Original} \\
    \multicolumn{1}{|l|}{($\phi=3$)} \bigstrut\\
    \hline
        \resultbf{89.43}
    \bigstrut\\
    \hline
        \result{99.71}
    \bigstrut\\
    \hline
        \resultbf{98.53}
    \bigstrut\\
    \hline
        \resultbf{99.70}
    \bigstrut\\
    \hline
        \result{96.21}
    \bigstrut\\
    \hline
        \result{99.50}
    \bigstrut\\
    \hline
        \result{89.20}
    \bigstrut\\
    \hline
        \resultbf{100.00}
    \bigstrut\\
    \hline
        \resultbf{100.00}
    \bigstrut\\
    \hline
        \result{95.72}
    \bigstrut\\
    \hline
        \result{99.08}
    \bigstrut\\
    \hline
        \resultbf{100.00}
    \bigstrut\\
    \hline
        \resultbf{98.46}
    \bigstrut\\
    % \hline
    \hhline{|=|}
        \resultbf{97.35}
    \bigstrut\\
    \hline
\end{tabular}
}


==> tables/old_unused/occl_5deg5cm_perobj.tex <==
% \begin{tabular}{|c||c|c|c||c|c|c||}
%     \hline
%     \multirow{2}{*}{Object}
%         & \multicolumn{3}{c||}{$\phi=0$}
%         & \multicolumn{3}{c||}{$\phi=3$} \\
%      \cline{2-7}
%     % Object
%          &
%          $\mathbb{P}^2$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\PY$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\PY$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
%         %     }
%         % }
%          &
%          $\mathbb{P}^2$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\PY$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\PY$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
%         %     }
%         % }
%          \\
%      \hline
%      ape
%         & \result{44.24}
%         & \result{49.29}
%         & \resultbf{56.87}
%         & \result{46.77}
%         & \result{46.67}
%         & \resultbf{62.63}
%         \\
%      \hline
%      can
%         & \result{79.41}
%         & \result{84.98}
%         & \resultbf{88.88}
%         & \result{82.63}
%         & \result{78.63}
%         & \resultbf{92.29}
%         \\
%      \hline
%      cat
%         & \result{77.50}
%         & \result{82.76}
%         & \resultbf{84.34}
%         & \result{79.78}
%         & \result{72.75}
%         & \resultbf{88.50}
%         \\
%      \hline
%      driller
%         & \result{88.85}
%         & \result{92.05}
%         & \resultbf{95.25}
%         & \result{92.24}
%         & \result{89.23}
%         & \resultbf{98.16}
%         \\
%      \hline
%      duck
%         & \result{52.92}
%         & \result{59.06}
%         & \resultbf{64.48}
%         & \result{57.60}
%         & \result{56.77}
%         & \resultbf{67.40}
%         \\
%      \hline
%      eggbox
%         & \result{35.41}
%         & \result{40.54}
%         & \resultbf{46.28}
%         & \result{53.22}
%         & \result{44.87}
%         & \resultbf{60.26}
%         \\
%      \hline
%      glue
%         & \result{56.77}
%         & \result{51.25}
%         & \resultbf{59.00}
%         & \result{59.40}
%         & \result{41.00}
%         & \resultbf{66.10}
%         \\
%      \hline
%      holepuncher
%         & \result{59.37}
%         & \result{63.31}
%         & \resultbf{69.82}
%         & \result{65.19}
%         & \result{63.41}
%         & \resultbf{75.25}
%         \\
%      \hline
%      Average
%         & \result{61.81}
%         & \result{65.40}
%         & \resultbf{70.61}
%         & \result{67.10}
%         & \result{61.67}
%         & \resultbf{76.32}
%         \\
%      \hline
% \end{tabular}


==> tables/old_unused/occl_reproj_perobj.tex <==
% \begin{tabular}{|c||c|c|c||c|c|c||}
%     \hline
%     \multirow{2}{*}{Object}
%         & \multicolumn{3}{c||}{$\phi=0$}
%         & \multicolumn{3}{c||}{$\phi=3$} \\
%      \cline{2-7}
%     % Object
%          &
%          Baseline
%         %  $\mathbb{P}^2$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\PY$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\PY$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\Hm_{\mathrm{aug}}$
%         %  $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
%         %     }
%         % }
%          &
%          Baseline
%         %  $\mathbb{P}^2$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\PY$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\PY$\\ Roll $180^\circ$
%         %     }
%         % }
%          &
%          $\Hm_{\mathrm{aug}}$
%         %  $\mathbb{P}^2$, Roll $45^\circ$, Tilt $20^\circ$
%         %  \rottableheader{
%         %     \parbox{3cm}{
%         %         $\mathbb{P}^2$\\ Roll $45^\circ$\\ Tilt $20^\circ$
%         %     }
%         % }
%          \\
%      \hline
%      ape
%         & \result{75.25}
%         & \result{75.96}
%         & \resultbf{80.61}
%         & \result{79.90}
%         & \result{78.28}
%         & \resultbf{86.87}
%         \\
%      \hline
%      can
%         & \result{89.85}
%         & \result{89.17}
%         & \resultbf{92.68}
%         & \result{89.46}
%         & \result{88.10}
%         & \resultbf{95.32}
%         \\
%      \hline
%      cat
%         & \result{85.83}
%         & \result{84.34}
%         & \resultbf{87.51}
%         & \result{88.21}
%         & \result{84.04}
%         & \resultbf{90.88}
%         \\
%      \hline
%      driller
%         & \result{88.85}
%         & \result{87.20}
%         & \resultbf{93.11}
%         & \result{90.11}
%         & \result{89.91}
%         & \resultbf{95.54}
%         \\
%      \hline
%      duck
%         & \result{78.75}
%         & \result{78.12}
%         & \resultbf{83.44}
%         & \result{81.77}
%         & \result{83.44}
%         & \resultbf{86.98}
%         \\
%      \hline
%      eggbox
%         & \result{54.73}
%         & \result{54.63}
%         & \resultbf{58.75}
%         & \result{61.77}
%         & \result{59.46}
%         & \resultbf{63.58}
%         \\
%      \hline
%      glue
%         & \result{68.99}
%         & \result{67.41}
%         & \resultbf{73.59}
%         & \resultbf{75.03}
%         & \result{65.57}
%         & \result{74.64}
%         \\
%      \hline
%      holepuncher
%         & \result{79.88}
%         & \result{82.45}
%         & \resultbf{87.48}
%         & \result{82.64}
%         & \result{83.53}
%         & \resultbf{90.34}
%         \\
%      \hline
%      Average
%         & \result{77.77} % Does not match 77.36??
%         & \result{77.41}
%         & \resultbf{82.15}
%         & \result{81.11}
%         & \result{79.04}
%         & \resultbf{85.52}
%         \\
%      \hline
% \end{tabular}

